Doubly-stochastic mining for heterogeneous retrieval

Modern retrieval problems are characterised by training sets with potentially billions of labels, and heterogeneous data distributions across subpopulations (e.g., users of a retrieval system may be from different countries), each of which poses a challenge. The first challenge concerns scalability: with a large number of labels, standard losses are difficult to optimise even on a single example. The second challenge concerns uniformity: one ideally wants good performance on each subpopulation. While several solutions have been proposed to address the first challenge, the second challenge has received relatively less attention. In this paper, we propose doubly-stochastic mining (S2M ), a stochastic optimization technique that addresses both challenges. In each iteration of S2M, we compute a per-example loss based on a subset of hardest labels, and then compute the minibatch loss based on the hardest examples. We show theoretically and empirically that by focusing on the hardest examples, S2M ensures that all data subpopulations are modelled well.

==> addendum.tex <==
% Recall that for random variable $\mathsf{U}$ and $\alpha \in (0, 1]$,
% the CVaR of $\mathsf{U}$ at level $\alpha$ is given by
% $$ \mathrm{CVaR}_\alpha( \mathsf{U} ) = \inf_{t \in \Real} \E{}{ \frac{1}{\alpha} [ \mathsf{U} - t ]_+ + t }. $$
% Further, recall that 
% for $\kExample = N \cdot \alpha$
% we used this to define the top-$\kExample$ risk of scorer $f \colon \XCal \to \Real$ via
% \begin{align*}
%     L_{\mathrm{top}( \kExample )}( f; \DCal ) &= \mathrm{CVaR}_\alpha( \mathsf{L}_f ) \\
%     &= \inf_{t \in \Real} \E{}{ \frac{1}{\alpha} [ \ell( \Y, f( \X ) ) - t ]_+ + t }.
% \end{align*}
% Following a similar analysis in~\citet{Boyd:2012} (see also~\citet[Proposition 1]{Duchi:2019}),
% we have the following Rademacher-based generalisation bound.

% %
% \begin{theorem}
% \label{thm:cvar-rademacher}
% Pick any $\delta \in (0, 1)$.
% Fix a function class $\FCal \subset \Real^{\XCal}$
% and 1-Lipschitz loss $\ell \colon [ \NumLabels ] \times \Real^{\NumLabels} \to \Real_+$
% with $B \defEq \| \ell \|_{\infty}$.
% Then, with probability at least $1 - \delta$ over a draw $S \sim \DCal^N$,
% for every $f \in \FCal$,
% $$ \mathrm{CVaR}_{\alpha}( \mathsf{L}_f; \DCal ) \leq \mathrm{CVaR}_{\alpha}( \widehat{\mathsf{L}}_f; \DCal ) + \frac{1}{\alpha} \cdot \left( \mathrm{Rad}_N( \FCal ) + \frac{B}{\sqrt{N}} \right) + \sqrt{\frac{\log \frac{1}{\delta}}{2N}} + \OCal\left( \frac{1}{\sqrt{N}} \right). $$
% \end{theorem}

% {\color{red}Let  $\Delta( \XCal \times [ \NumLabels ] )$ be the set of all distributions over $\XCal \times [\NumLabels ]$. Equipped with Theorem~\ref{thm:cvar-rademacher},}
% we may now appeal to a distinct representation for the CVaR,
% which yields the following
% bound
% on the loss
% over \emph{all} subpopulations of fraction at least $\alpha$.
% A similar connection between the CVaR and subpopulation losses was made in~\citet[Equation 2]{Duchi:2019}.

% %
% \begin{corollary}
% \label{corr:subpopulation-control}
% Pick any $\delta \in (0, 1)$.
% Fix a function class $\FCal \subset \Real^{\XCal}$
% and 1-Lipschitz loss $\ell \colon [ \NumLabels ] \times \Real^{\NumLabels} \to \Real_+$
% with $B \defEq \| \ell \|_{\infty}$.
% Then, with probability at least $1 - \delta$ over a draw $S \sim \DCal^N$,
% for every $f \in \FCal$,
% $$ \sup_{\bar{\DCal} \in \mathscr{U}_\alpha( \DCal )} \E{( \X, \Y ) \sim \bar{\DCal}}{ \ell( \Y, f( \X ) ) } \leq \mathrm{CVaR}_{\alpha}( \widehat{\mathsf{L}}_f; \DCal ) + \frac{1}{\alpha} \cdot \left( \mathrm{Rad}_N( \FCal ) + \frac{B}{\sqrt{N}} \right) + \sqrt{\frac{\log \frac{1}{\delta}}{2N}} + \OCal\left( \frac{1}{\sqrt{N}} \right), $$
% where $\mathscr{U}_\alpha$ comprises all subpopulations of size at least $\alpha$:
% $$ \mathscr{U}_\alpha( \DCal ) = \{ \bar{\DCal} \in \Delta( \XCal \times [ \NumLabels ] ) \mid \exists \bar{\DCal}' \in \Delta( \XCal \times [ \NumLabels ] )~\text{such that}~\DCal = \alpha \cdot \bar{\DCal} + (1 - \alpha) \cdot \bar{\DCal}' \}. $$
% \end{corollary}

%
\begin{proof}[Proof of Theorem~\ref{thm:cvar-rademacher}]
Define
$$ L_{\alpha}( f, t; \DCal ) \defEq \E{}{ \frac{1}{\alpha} [ \ell( \Y, f( \X ) ) - t ]_+ + t }. $$
We thus have $L_{\mathrm{top}( \kExample )}( f; \DCal ) = L( f, t^*; \DCal )$ where $t^*$ is the $(1 - \alpha)$th quantile of the loss values.
We similarly have the empirical version
$$ \hat{L}_{\alpha}( f, t; S ) \defEq \frac{1}{N \alpha} \sum_{n = 1}^N [ \ell( \Y, f( \X ) ) - t ]_+ + t. $$

For $\bar{\ell}_{\alpha, t}( y, f ) \defEq \frac{1}{\alpha} [ \ell( y, f ) - t ]_+ + t$,
we may write
$$ L( f, t; \DCal ) = \E{}{ \bar{\ell}_{\alpha, t}( \Y, f( \X ) ) }, $$
and similarly for the empirical version.
Consequently, a standard analysis yields that with probability at least $1 - \delta$,
$$ L( f, t; \DCal ) \leq \hat{L}( f, t; S ) + 2 \cdot \mathrm{Rad}_N( \bar{\FCal}_{t} ) + \sqrt{\frac{\log \frac{1}{\delta}}{2N}}, $$
where 
%$\bar{\FCal}_{\alpha, t} \defEq \{ \bar{\ell}_{\alpha, t} \circ f \colon f \in \FCal, t \in [ 0, B ] \}$.
$\bar{\FCal}_{\alpha} \defEq \{ ( x, y ) \mapsto \bar{\ell}_{\alpha, t}( y, f( x ) ) \colon f \in \FCal, t \in [ 0, B ] \}$.

The function $z \mapsto \frac{1}{\alpha} \cdot [ z ]_+$ is clearly $\frac{1}{\alpha}$-Lipschitz,
and so by the contraction principle,
$\mathrm{Rad}_N( \bar{\FCal}_{\alpha} ) \leq \frac{1}{\alpha} \cdot \mathrm{Rad}_N( \tilde{\FCal} )$,
where
$\tilde{\FCal} \defEq \{ ( x, y ) \mapsto \ell( y, f( x ) ) - t \colon f \in \FCal, t \in [ 0, B ] \}$.
Following~\citet[Theorem 1]{Boyd:2012},
we have that $\mathrm{Rad}_N( \tilde{\FCal} ) \leq \mathrm{Rad}_N( {\FCal}_{\ell} ) + \frac{B}{\sqrt{N}}$,
for 
${\FCal}_{\ell} \defEq \{ ( x, y ) \mapsto \ell( y, f( x ) ) \colon f \in \FCal \}$.
Applying the contraction principle once more,
by the assumption that $\ell$ is 1-Lipschitz,
$\mathrm{Rad}_N( {\FCal}_{\ell} ) \leq \mathrm{Rad}_N( {\FCal} )$.
It thus follows that for every $f \in \FCal$ and $t \in [ 0, B ]$,
$$ L_{\alpha}( f, t; \DCal ) \leq \hat{L}_{\alpha}( f, t; S ) + \frac{1}{\alpha} \cdot \left( \mathrm{Rad}_N( \FCal ) + \frac{B}{\sqrt{N}} \right) + \sqrt{\frac{\log \frac{1}{\delta}}{2N}}. $$

Since the above holds uniformly for every $t \in [ 0, B ]$,
we may plug in $t$ to be the population-level loss quantile.
For the right hand side, one may bound this ({\color{red}following the steps in the proof of Corollary~\ref{corr:top-k}})
by the choice of the empirical quantile,
plus the deviation between the empirical and true quantile.
Thus, we arrive at
$$ \mathrm{CVaR}_{\alpha}( \mathsf{L}_f; \DCal ) \leq \mathrm{CVaR}_{\alpha}( \widehat{\mathsf{L}}_f; \DCal ) + \frac{1}{\alpha} \cdot \left( \mathrm{Rad}_N( \FCal ) + \frac{B}{\sqrt{N}} \right) + \sqrt{\frac{\log \frac{1}{\delta}}{2N}} + \OCal\left( \frac{1}{\sqrt{N}} \right). $$
\end{proof}


%
\begin{proof}[Proof of Corollary~\ref{corr:subpopulation-control}]
We use the following representation of the CVaR~\citep[Example 4.2]{BenTal:2007}:
for random variable $\mathsf{U} \colon \Omega \to U$
defined over probability space $( \Omega, \Sigma, P )$,
\begin{align*}
\mathrm{CVaR}_{\alpha}( \mathsf{U} ) &= \sup_{Q \in \mathscr{U}_\alpha( P )} \E{\mathsf{U}' \sim Q}{ \mathsf{U}' } \\
\mathscr{U}_\alpha( P ) &= \{ Q \in \Delta( U ) \mid P( A ) \geq \alpha \cdot Q( A ),~\forall A \in \Sigma\}.
\end{align*}
The CVaR is thus the maximal expectation of the random variable 
under any distribution from an uncertainty set $\mathscr{U}_\alpha( P )$.
This uncertainty set considers all distributions for which the probability measure cannot deviate too far from the original, in the sense of the ratio of the measures being bounded.
We may rewrite this as (see also the related notion of mutual irreducibility in~\citet{Scott:2013})
$$ \mathscr{U}_\alpha( P ) = \{ Q \in \Delta( U ) \mid \exists R \in \Delta( U )~\text{such that}~P = \alpha \cdot Q + (1 - \alpha) \cdot R \}. $$
That is, the uncertainty set comprises all \emph{minority subpopulations} of the original distribution,
which have mass at least $\alpha$.
Consequently,
$$ \sup_{\bar{\DCal} \in \mathscr{U}_\alpha( \DCal )} \E{( \X, \Y ) \sim \bar{\DCal}}{ \ell( \Y, f( \X ) ) } \leq \mathrm{CVaR}_{\alpha}( \widehat{\mathsf{L}}_f; \DCal ) + \frac{1}{\alpha} \cdot \left( \mathrm{Rad}_N( \FCal ) + \frac{B}{\sqrt{N}} \right) + \sqrt{\frac{\log \frac{1}{\delta}}{2N}} + \OCal\left( \frac{1}{\sqrt{N}} \right), $$
so that we can bound the worst-case expected loss
over all subpopulations of fraction at least $\alpha$.
\end{proof}


==> related.tex <==
Our work leverages ideas from several works, including learning from large number of samples, large number of labels, and learning to ensure consistent performance across sub-populations of the data.
We review some relevant works from each of these areas.

%
\textbf{Large-scale learning}.
Stochastic gradient descent~\citep{Robbins:1951} is the \emph{de facto} approach to training models with large numbers of instances.
In its simplest form, one samples a \emph{minibatch} of $B$ examples at each iteration, and performs a descent step based on the corresponding loss on the minibatch.
When $B \ll N$, SGD makes training with a large number of samples tractable.
Recent years have seen study of a  number of practically important extensions of SGD,
such as means of reducing the variance of the gradient estimates~\citep{Johnson:2013,Defazio:2014,Zhao:2015},
adaptively tuning learning rates~\citep{Duchi:2011,Adam:2015,Reddi:2018},
and making the updates feasible in a distributed setting~\citep{Zinkevich:2010,Dean:2012,McMahan:2017}.


%
\textbf{Extreme classification}.
Extreme classification is the common real-world problem of multiclass classification with a large number of classes~\citep{Agrawal:2013,Yu:2014,Bhatia:2015,Jain:2016,Babbar:2017,Yen:2017,Prabhu:2018,Jain:2019}.
This poses a challenge for SGD, since even \emph{computing} the full minibatch loss may be prohibitive, let alone optimising it.

One approach to cope with this problem is to \emph{sample} the set of labels, and use a resulting stochastic approximation to the loss.
A canonical example is the sample softmax~\citep{Bengio:2008,Blanc:2018},
which exhibits good performance, potentially at the expense of some bias.
For more general losses,
a simple strategy is to randomly sample negatives~\citep{Mikolov:2013}.

\citet{Reddi:2019} proposed stochastic negative mining (SNM),
which operates by randomly sampling a batch of labels, and then retaining only those which are maximally confused with the true label.
(See~\S\ref{sec:snm} for mathematical details.)
This may be related to hard negative mining, which in batch settings retains samples that are maximally difficult for the model~\citep{Sung:1996,Dalal:2005,Felzenszwalb:2010,Shrivastava:2016}.
Other forms of ``difficulty-based'' example and label sampling have also been explored~\citep{Mineiro:2013,Schroff:2015,Bai:2017}.

%
\textbf{Max- and top-$k$ loss}.
Standard empirical risk minimisation proposes to minimise the average loss over the training sample.
One may replace the average with other summary statistics,
with the hope of for example obtaining better generalisation~\citep{Chapelle:2000,Maurer:2009}.
A natural alternate candidate
is 
the \emph{maximum} loss over the sample.
In the case of the hinge loss, this corresponds to the hard-margin SVM~\citep{Vapnik:1999}.
For more general losses, 
% the maximal loss may be useful to control the risk over subpopulations of the data.
\citet{Shalev-Shwartz:2016} propose to minimise the maximal loss over all samples, and show that this can guarantee good performance on data sub-populations.

%
The maximum loss may be vulnerable to outliers.
A more conservative choice is thus the \emph{top-$k$ loss},
which only considers the average of the top-$k$ largest scoring instances.
\citet{Yang:2014} proposed a ``coherent'' loss which is the average of the top-$k$ risks, where $k$ is chosen so as to satisfy certain axioms.
\citet{Fan:2017} propose to minimise the average of the top-$k$ largest losses, motivated by class-imbalance and outlier samples.
\citet{Kawaguchi:2019} propose a stochastic analogue of this method, which computes the average of the top-$k$ largest losses in a minibatch.

%
A related line of work has explored the use of the average of the top-$k$ \emph{subgroup risks},
so as to ensure a form of fairness~\citep{Alabi:2018,Mohri:2019,Williamson:2019}.
Informally, these seek to ensure that each subgroup of the data incurs similar loss.
Typically, one assumes that the subgroup membership of each instance is known;
when this is not true,
one may nonetheless guard against worst-case subgroup assignments via a form of robust optimisation~\citep{Hashimoto:2018}.

%
% We remark here that minimising the \emph{smallest} losses,
% also known as a \emph{trimmed} average,
% has a rich history in robust statistics~\citep{Rousseeuw:1987,Bhatia:2015b,Yang:2018}.
% In a learning context,~\citet{Shen:2019} proposed to minimise the smallest-$k$ losses to endow models with robustness.
% AKM: no need to mention this as it's a different topic, that just happens to use a similar loss.
% \citet{Ghadikolaei:2019} {\color{red} also!!!} propose an iterative algorithm which minimises the smallest-$k$ losses at every iteration.

% %
% \textbf{Other work}.
% \citet{Feldman:2019} considered the issue of memorisation versus generalisation, including an analysis of learning on a mixture of subpopulations.
% \citet{Herath:2019} considered a maximal discrepancy objective in the context of transfer learning.
% Our approach is distinct from doubly stochastic gradient descent as used in kernel methods~\citep{Dai:2014}.


==> toolbox.tex <==
\begin{theorem}[\bf Contraction principle \cite{LedT13}]
\label{thm:contraction}
Let $\varepsilon_1, \varepsilon_2,\ldots, \varepsilon_d$ be $d$ independent Rademacher RVs and  $f: \R_{+} \to \R_{+}$ be a convex and increasing function. Let $\phi_{i}:\R \rightarrow \R$ be an $L$-Lipschitz function, i.e.,
$|\phi_i(a) - \phi_i(b)| \leq L |a - b|,$
which satisfy $\phi_i(0) = 0$. Then, for any $T \subseteq \R^d$, 
\begin{align}
\E{}{f\left(\frac{1}{2} \sup_{t \in T} \Big\vert \sum_{i = 1}^{d} \varepsilon_i \phi_i(t_i)\Big\vert \right)} \leq \E{}{ f \left(L \cdot \sup_{t \in T}\Big\vert \sum_{i = 1}^{d}\varepsilon_it_i\Big\vert\right)}.
\end{align}
\end{theorem}

\begin{lemma}
Assume that the loss function $\ell : \YCal \times \Real^L \to \Real$ satisfies the condition:
\begin{align}
\|\ell(y, u) - \ell(y, v)\|_2 \leq \gamma \|u - v \|_2.
\end{align}
Then $f \mapsto \widehat{C}_{\alpha}(\ell(Y,f(X)))$ and $f \mapsto \cvar_{\alpha}(\ell(Y,f(X)))$ are Lipschitz functions over the set $\FCal$ with constant $\frac{\gamma}{\alpha}$, i.e.,
\begin{align}
\big\|\widehat{C}_{\alpha}(\ell(Y,f(X))) - \widehat{C}_{\alpha}(\ell(Y,f'(X)))\big\|_2 \leq \frac{\gamma}{\alpha}\|f - f'\| \\
\big\|\cvar_{\alpha}(\ell(Y,f(X))) - \cvar_{\alpha}(\ell(Y,f'(X)))\big\|_2 \leq \frac{\gamma}{\alpha}\|f - f'\|
\end{align}
\end{lemma}

